Co-segmentation for Space-Time Co-located Collections

We present a co-segmentation technique for space-time co-located image collections. These prevalent collections capture various dynamic events, usually by multiple photographers, and may contain multiple co-occurring objects which are not necessarily part of the intended foreground object, resulting in ambiguities for traditional co-segmentation techniques. Thus, to disambiguate what the common foreground object is, we introduce a weakly-supervised technique, where we assume only a small seed, given in the form of a single segmented image. We take a distributed approach, where local belief models are propagated and reinforced with similar images. Our technique progressively expands the foreground and background belief models across the entire collection. The technique exploits the power of the entire set of image without building a global model, and thus successfully overcomes large variability in appearance of the common foreground object. We demonstrate that our method outperforms previous co-segmentation techniques on challenging space-time co-located collections, including dense benchmark datasets which were adapted for our novel problem setting.

==> comparison_davis.tex <==
\section{Results and comparisons on sampled video collections}
In Figure \ref{fig:davis1} %and Figure \ref{fig:davis2} 
we provide additional qualitative results and comparisons on the first five frames from the sparse sequences sampled from the Davis datasets \cite{Perazzi2016}. See Table 1 in the paper for a quantitative evaluation on these datasets.

\begin{figure*}
\vspace{-5pt}

\footnotesize
	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{rubinstein2013unsupervised}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/boat_1.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/soapbox_1.png}	\\
	\vspace{-16pt}

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{faktor2013co}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/boat_2.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/soapbox_2.png}	\\
	
	\vspace{-16pt}
	
	\rotatebox[origin=c]{90}{\whitetxt{2222}  \cite{kim2012multiple}}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/boat_3.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/soapbox_3.png}	\\
		
	\vspace{-16pt}	
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/boat_4.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/soapbox_4.png}	\\

	\vspace{-14pt}	

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{rubinstein2013unsupervised}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/lucia_1.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/drift-turn_1.png}	\\
	\vspace{-16pt}

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{faktor2013co}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/lucia_2.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/drift-turn_2.png}	\\
	
	\vspace{-16pt}
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{kim2012multiple}}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/lucia_3.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/drift-turn_3.png}	\\
		
	\vspace{-16pt}	
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/lucia_4.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/drift-turn_4.png}	\\

	\vspace{-14pt}	

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{rubinstein2013unsupervised}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/rhino_1.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/stroller_1.png}	\\
	\vspace{-16pt}

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{faktor2013co}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/rhino_2.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/stroller_2.png}	\\
	
	\vspace{-16pt}
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{kim2012multiple}}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/rhino_3.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/stroller_3.png}	\\
		
	\vspace{-16pt}	
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/rhino_4.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/stroller_4.png}	\\

	\vspace{-14pt}	

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{rubinstein2013unsupervised}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-walk_1.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_1.png}	\\
	\vspace{-16pt}

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{faktor2013co}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-walk_2.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_2.png}	\\
	
	\vspace{-16pt}
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{kim2012multiple}}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-walk_3.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_3.png}	\\
		
	\vspace{-16pt}	
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-walk_4.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_4.png}	\\

	\vspace{-14pt}	

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{rubinstein2013unsupervised}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/parkour_1.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/motorbike_1.png}	\\
	\vspace{-16pt}

	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{faktor2013co}}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/parkour_2.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/motorbike_2.png}	\\
	
	\vspace{-16pt}
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} \cite{kim2012multiple}}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/parkour_3.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/motorbike_3.png}	\\
		
	\vspace{-16pt}	
	
	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/parkour_4.png} 
\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/motorbike_4.png}	\\


\vspace{-10pt}
%\small
	\caption{Qualitative comparison to state-of-the-art co-segmentation techniques on the first five frames from the sparse sequences sampled from the following Davis datasets \cite{Perazzi2016}: boat, soapbox, lucia, drift-turn, rhino, stroller, kite-walk, scooter-black, parkour, motorbike. The first frame is provided as template for the semi-supervised techniques.
}
	\label{fig:davis1}
\end{figure*}

%\begin{figure*}
%\vspace{-5pt}
%
%\footnotesize
%	\rotatebox[origin=c]{90}{\whitetxt{2222} RJKL13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/car-roundabout_1.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-surf_1.png}	\\
%	\vspace{-20pt}
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} FI13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/car-roundabout_2.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-surf_2.png}	\\
%	
%	\vspace{-14pt}
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} KX12}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/car-roundabout_3.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-surf_3.png}	\\
%		
%	\vspace{-16pt}	
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/car-roundabout_4.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/kite-surf_4.png}	\\
%
%	\vspace{-14pt}	
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} RJKL13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/tennis_1.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/hike_1.png}	\\
%	\vspace{-20pt}
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} FI13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/tennis_2.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/hike_2.png}	\\
%	
%	\vspace{-14pt}
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} KX12}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/tennis_3.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/hike_3.png}	\\
%		
%	\vspace{-16pt}	
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/tennis_4.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/hike_4.png}	\\
%
%	\vspace{-14pt}	
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} RJKL13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/swing_1.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_1.png}	\\
%	\vspace{-20pt}
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} FI13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/swing_2.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_2.png}	\\
%	
%	\vspace{-14pt}
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} KX12}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/swing_3.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_3.png}	\\
%		
%	\vspace{-16pt}	
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/swing_4.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/scooter-black_4.png}	\\
%
%	\vspace{-14pt}	
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} RJKL13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/goat_1.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/camel_1.png}	\\
%	\vspace{-20pt}
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} FI13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/goat_2.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/camel_2.png}	\\
%	
%	\vspace{-14pt}
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} KX12}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/goat_3.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/camel_3.png}	\\
%		
%	\vspace{-16pt}	
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/goat_4.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/camel_4.png}	\\
%
%	\vspace{-14pt}	
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} RJKL13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/horsejump-high_1.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/car-turn_1.png}	\\
%	\vspace{-20pt}
%
%	\rotatebox[origin=c]{90}{\whitetxt{2222} FI13}   \hfill \includegraphics[width=0.47\textwidth]{figures/DAVIS/horsejump-high_2.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/car-turn_2.png}	\\
%	
%	\vspace{-14pt}
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} KX12}   \hfill  \includegraphics[width=0.47\textwidth]{figures/DAVIS/horsejump-high_3.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/car-turn_3.png}	\\
%		
%	\vspace{-16pt}	
%	
%	\rotatebox[origin=c]{90}{\whitetxt{2222} Ours}   \hfill    \includegraphics[width=0.47\textwidth]{figures/DAVIS/horsejump-high_4.png} 
%\includegraphics[width=0.47\textwidth]{figures/DAVIS/supp/car-turn_4.png}	\\
%
%
%\vspace{-10pt}
%%\small
%	\caption{Qualitative comparison to state-of-the-art co-segmentation techniques on the first five frames from the sparse sequences sampled from the following Davis datasets \cite{Perazzi2016}: car-roundabout, kite-surf, tennis, hike, swing, scooter-black, goat, camel, horsejump-high, and car-turn.  The first frame is provided as template for the semi-supervised techniques.
%}
%	\label{fig:davis2}
%\end{figure*}


==> inference_evaluation.tex <==
\section{Evaluating our inference technique}
 \label{sec:evaluation}
 
To evaluate our inference technique, we provide both qualitative and quantitative results on the following intermediate stages: (i) single inference from correspondences only;   (ii) a complete direct template-target inference application; and (iii) joint multi-target inference.
In Table \ref{tab:comp}(a), we report the average $P$ and $J$ scores per dataset. These scores average over all the images which are adjacent to a template seed, and further average over three random template seeds per dataset.
To evaluate how well the correspondences provided by NRDC capture the object in the target images, we report two different scores. The first (indicated by (i) in Table \ref{tab:comp}(a)) considers foreground regions directly according to the foreground correspondences. The yellow regions in Figure \ref{fig:stages} illustrate these regions. The second (indicated by (i)+ in Table \ref{tab:comp}(a)) considers foreground regions that are obtained after performing graph-cuts, with these regions provided for initialization. %We also report the scores obtained from a complete single inference application (indicated by (ii) in Table \ref{tab:comp}(a)) and from a joint multi-target inference (indicated by (iii) in Table \ref{tab:comp}(a)).

As can be observed both in Table \ref{tab:comp}(a) and Figure \ref{fig:stages}, our technique achieves a significant improvement over the initial set of reliable correspondences.
Note that our technique is robust a to few outliers (false positives), e.g., in the right-most image of Figure \ref{fig:stages}, and recovers the object thanks to the joint multi-target inference stage. For a more extensive assessment of our inference technique, please refer to the interactive html files.

\begin{figure*}[t]
\vspace{-20pt}
	\includegraphics[width=0.245\textwidth]{figures/inference_stages/Set1/im_num3.png}
	\includegraphics[width=0.245\textwidth]{figures/inference_stages/Set1/im_num7.png}
	\includegraphics[width=0.245\textwidth]{figures/inference_stages/Set1/im_num10.png}
	\includegraphics[width=0.245\textwidth]{figures/inference_stages/Set1/im_num12.png}

	
	\vspace{-8pt}
	\caption{Comparison to the correspondences provided by NRDC. For each template-target image pair, the reliable correspondences are colored in either yellow (in foreground regions) or blue (in background regions). The silhouettes of our multi-target inference results are provided in red. %As the figure illustrates, we can successfully segment the object from only partial object matches or even from false matches, as the right-most image in the top row demonstrates.  
}
\label{fig:stages}
\end{figure*}


\begin{table}[t]
\centering
%\begin{subtable}{.5\textwidth}

%\resizebox{\columnwidth}{!}{%
\centering%\footnotesize
\vspace{-10pt}
\ra{0.6}
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{@{}lllrcrrrrrr@{}}
\toprule
\multicolumn{2}{c}{} &  & \multicolumn{2}{c}{\textsc{Bride}} & \phantom{}& \multicolumn{2}{c}{\textsc{Singer}} & \phantom{} & \multicolumn{2}{c}{\textsc{Toddler}}\\
%\cmidrule{1-3} \cmidrule{5-5} \cmidrule{7-8} \cmidrule{10-11}
 && & P & J &&  P & J &&  P & J \\ \midrule
 (i) && & 66.6 & 16.2 && 78.2 & 09.1  && 92.0 & 37.6 \\ %Rubinstein et al. 
 (i)+ && & 68.5 & 19.8 && 77.8 & 11.5  && 93.6 & 47.1 \\ %Faktor et al. 
 (ii) && & 89.4 & 78.9 && 97.2 & 88.6  && 96.3 & 75.0 \\ %Kim et al. 
 (iii) && & \textbf{92.2} & \textbf{83.0}  && \textbf{98.4} & \textbf{93.8} && \textbf{96.9} & \textbf{79.9}\\

%Name & \#img & \#ppl && && $1$D & $2$D && 1\hspace{5pt} & 2\hspace{5pt} \\ \midrule
%\emph{$1^{st}$ Setting:}\\
%\textsc{Headstand} &11 &11 && 0 && 10 & 0 && 6* & 7* \\
\bottomrule
\end{tabular}
%}
\vspace{-3pt}
\caption{\textbf{Evaluation of our inference approach}. We break-down the performance of the different stages (numbered according to Section \ref{sec:evaluation}) of a single inference iteration. 
 \label{tab:comp}
\vspace{-8pt}
}
\end{table}

==> overview.tex <==
% !TEX root =  seg-eccv.tex 


%\begin{figure}[t]
%	\vspace{-10pt}
%	\includegraphics[width=\columnwidth]{figures/graph_2.pdf}
%	\vspace{-10pt}
%	\caption{Propagating local belief models to images which are adjacent to the current seed. The object likelihood maps of the adjacent images (in purple) are first inferred from the seed (in orange) separately, and then these initial estimates are reinforced and refined. From the refined estimates, we extract the common foreground objects (in red).    
%%	At each step, 
%%	we jointly infer the beliefs of all the parts belonging to the adjacent images (in purple) of our current seed image (in orange). From these local beliefs, we extract the common foreground objects (marked in red). Continuing with a new seed, we repeat these interleaving steps until convergence. 	
%}
%	\label{fig:image_graph}
%\end{figure}


\section{Overview} 

% Input and goal, mention why we require a template.

Given a collection of space-time co-located images, our method co-segments the images and extracts a common foreground object. 
Since this task is ambiguous, we ask the user to provide a manually segmented template image to specify what the common object is.

% Distributed approach

The foreground object varies considerably in appearance across the entire collection.
Thus, we do not use a single global model to represent it, but instead take a distributed approach.
We decompose each image into parts at multiple scales.
Parts store local beliefs about the foreground and background models.
These beliefs are propagated to similar parts within and among images.
In each iteration, one image is selected as a current seed.
The details of the algorithm are described in Section~\ref{sec:iterations}.

% Propagation

The propagation itself is formulated as a convex belief propagation (CBP) optimization. 
We provide brief background on CBP in Section~\ref{sec:background}.
In Section~\ref{sec:single} we describe how to infer the object likelihood map of a single target image from a given seed image.
In Section \ref{sec:multiopt}, we then introduce how the initial likelihood estimates can be refined and reinforced from multiple target images.

%At each step, an image is defined as a seed (highlighted in orange in Figure \ref{fig:image_graph}). We then analyze the seed in a number of scales, generating a large bag of segments representing candidate parts to learn from. These multilevel parts represent the foreground and background models from which target parts of adjacent images infer their likelihood to be labeled as either foreground or background. This key idea is illustrated in Figure \ref{fig:parts_unary}, where corresponding parts are marked with similar colors. As we will elaborate more in Section \ref{sec:single}, each target patch can be associated with a single patch in the augmented bag of patches. 

%We expand the seed model to more images in the collection while repeatedly using convex belief propagation. A single application of convex belief propagation, which grows the seed inside an image, amounts to passing messages within the image to create local probability distributions over the image parts. These local probability distributions are the beliefs and the convex belief propagation algorithm enforces consistencies among beliefs that share the same parts. We also pass beliefs among images (see illustration in Figure \ref{fig:image_graph}). This step introduces novel non-linearities to the inference process that encourage part beliefs across images to be similar. We use variational inference approach to guarantee that these two optimization components are tied by a single global optimum using convex analysis.   

%\hadar{The inference of the object forms likelihood maps which are refined progressively with a series of message passing steps among similar images. Starting from a given seed segmentation, the information is iteratively propagated over to the collection using the labeling estimates of the collection images. Inference is performed from a current seed outward, where the probabilities of parts to be associated with parts in similar images are first inferred within each image separately, and then the probabilities of parts are propagated across images to reinforce consistent probabilities over all parts. }

%The rest of the paper is organized as follows: For completeness, we first present preliminaries on convex belief propagation optimization in Section \ref{sec:background}. Then in Section \ref{sec:single}, we detail how to infer the object likelihood maps of a single target image from a given seed. In Section \ref{sec:multiopt} we introduce how the initial likelihood estimates can be refined and reinforced from multiple target images. Finally, in Section \ref{sec:iterations}, we present the full co-segmentation framework. 
%detail about the image-graph construction and iteration between learning the likelihood estimates and co-segmenting the images. 
%In Section \ref{sec:evaluation} we present results and conclude in Section \ref{sec:conclusions}.


==> potentials.tex <==

\hadar{Obsolete:

\section{Two-stage optimization}
In each propagation step, we pass the beliefs of the current template to its neighbors in two stages. First, we consider each neighbor separately and construct appropriate template-neighbor potentials $\theta_i,\theta_{i,j}$ and maximize Equation \ref{eq:cbp} to obtain a confidence measure per part $b_i$. Then, these measures become our unary terms for a joint neighbors optimization. In what follows, we first elaborate on the potentials $\theta_i,\theta_{i,j}$ that we consider for the first stage (Section \ref{sec:firststage}) and then detail the second step and prove its optimality? (Section \ref{sec:secondstage}). 

\subsection{Template-neighbor potentials} \label{sec:firststage}

\paragraph{Unary potentials}

Normally unary potentials describe the degree of which a pixel, or a part, agrees with the foreground or background models. In our setting, the inherent image models are completely latent. We do, however, have foreground and background labellings of our source image from which we would like to infer these potentials.     

From the labellings of the source image, we construct a foreground and background model which is composed of all the corresponding image parts. More precisely, let $s_1=\{s^i_1 \}$ and $s_0=\{s^i_0 \}$ represent our foreground and background models, where $s^i_1$ and $s^i_0$ are the different labelled parts. To obtain parts, we use the hierarchical segmentation method of \cite{arbelaez2011contour} at multiple scales/thresholds $\{T\}$. 

For each part $t_j$ in the target image, derived from the method of \cite{arbelaez2011contour} with $T=0.08$, we define its unary potentials as follows:
\begin{equation}
\theta_{t_j} =  \max_{s^i_1}\  p_{corr}(s^i_1,t_j)  - \max_{s^i_0}\  p_{corr}(s^i_0,t_j),
\end{equation}

%where
%
%\begin{equation} 
%p^*_{corr}(s^i_1,t_j)= \left\{
%\begin{array}{cc}
% p_{corr}(s^i_1,t_j) & \text{if } p_{corr}(s^i_1,t_j)>0 \\
% \lambda p_{sim}(s^i_1,t_j) & \text{otherwise},
%\end{array}\right.
%\end{equation}


%We shall begin by describing $p_{corr}$ and then explain the extension to $p^*_{corr}$ for the foreground labelled parts. 
%Note that $\lambda=0.1$ is a balancing coefficient, $p_{corr}$ is the probability of which the two parts correspond, and $p_{sim}$ describes how similar the two parts are.

We compute $p_{corr}(p_1,p_2)$ as follows: 
\begin{equation}
p_{corr}(p_1,p_2) = \frac{N(p_1,p_2)}{ m_{p_2}},
\end{equation}

where $N(p_1,p_2)$ is the number of matching pixels and $m_{p_2}$ is the overall count of pixels in $p_2$. To compute matching pixels, we use the dense correspondence technique of Yoav Ha-Cohen et al. \cite{hacohen2011non} which outputs a confidence value along with the pixel-to-pixel correspondences. We consider matching pixels to be those with confidence values which exceed a certain threshold, which we set empirically to $0.5$. As Figure \ref{fig:NRDC} demonstrates, this yields a rather sparse set of clean correspondences. While other approaches may yield a larger set of correspondences, here we care for precision, or only a small number of false-positive approximate correspondences. 

\paragraph{Pairwise Potentials}

We have two types of pairwise potentials between two different parts in each neighboring image - $\theta^{source}_{t_i,t_j}$ and $\theta^{sim}_{t_i,t_j}$.

We shall start by defining $\theta^{source}_{t_i,t_j}$ which aims at locating more commonality to the source image than what is evident by the given correspondences. For each source part $s^i_1$, we compute an RGB color histogram and find the $K$ closest parts in the target. We then look at two adjacents parts in the source image and check whether their corresponding parts are also adjacent. If so, we define a pairwise relation as follows:
\begin{equation}
\theta^{source}_{t_i,t_j} = ....
\end{equation}

Rather than allowing any two parts to correspond, we can propagate knowledge from the given pixel correspondences by estimating where the corresponding part in the target should be. We can do so in the following manner: For each part $s^i_1$, we find the closest and furthest foreground corresponding pixels and approximate the location of the corresponding part according to its relative location. We then allow for an uncertainty gap by setting an uncertainty radius according to the distance from the closest correspondence. See Figure \ref{fig:NRDC2} for an illustration.
%We examine if any of the $K$ closest neighbors reside within this \emph{uncertainty area} and update $p_{sim}(s^i_1,t_j)$ accordingly only if one of the $K$ nearest neighbors of one of the template's spatial neighbors is bordering with $t_j$. In other words, we consider target parts that are similar to template parts in pairs. Like with the correspondences, this yields a conservative but highly reliable set....To densify our estimations, we use weaker cues for template foreground parts that have no corresponding pixels. 

Another type of inter-image potential is $\theta^{sim}_{t_i,t_j}$ which measures how likely the two parts coincide, according to the hierarchical segmentation of \cite{arbelaez2011contour}. As parts are defined according to the different thresholds, we can sample various thresholds to compute the likelihood in which two parts will become one according to this method. More precisely, we define a pairwise relation between adjacent parts in each target image according to:
\begin{equation}
\theta^{sim}_{t_i,t_j} = ....
\end{equation}


\subsection{Joint neighbors optimization} \label{sec:secondstage}

\paragraph{Unary potentials} As detailed earlier, the confidence measures  $b_i$ serve as our unary potentials in this stage.

\paragraph{Pairwise potentials}
Pairwise connections between neighbouring images are defined according to the degree of which they correspond. As the dense correspondence technique we use is not symmetric, we define these connections as follows:
\begin{equation}
\theta^{corr}_{t_i,t_j} = \frac{N(t_i,t_j)}{ m_{t_i}}+\frac{N(t_j,t_i)}{ m_{t_j}},
\end{equation}

where $N(t_i,t_j)$ is the number of matching pixels from part $t_i$ to $t_j$ and $m_{t_i}$ is the overall count of pixels in $t_i$.

}

==> potentialsOneStep.tex <==
\section{Unary potentials}

Normally unary potentials describe the degree of which a pixel, or a part, agrees with the foreground or background models. In our setting, the inherent image models are completely latent. We do, however, have foreground and background labellings of our source image from which we would like to infer these potentials.     

From the labellings of the source image, we construct a foreground and background model which is composed of all the corresponding image parts. More precisely, let $s_1=\{s^i_1 \}$ and $s_0=\{s^i_0 \}$ represent our foreground and background models, where $s^i_1$ and $s^i_0$ are the different labelled parts. To obtain parts, we use the hierarchical segmentation method of \cite{arbelaez2011contour} at multiple scales/thresholds $\{T\}$. 

For each part $t_j$ in the target image, derived from the method of \cite{arbelaez2011contour} with $T=0.08$, we define its unary potentials as follows:
\begin{equation}
\theta_{t_j} =  \max_{s^i_1}\  p_{corr}(s^i_1,t_j)  - \max_{s^i_0}\  p_{corr}(s^i_0,t_j),
\end{equation}

%where
%
%\begin{equation} 
%p^*_{corr}(s^i_1,t_j)= \left\{
%\begin{array}{cc}
% p_{corr}(s^i_1,t_j) & \text{if } p_{corr}(s^i_1,t_j)>0 \\
% \lambda p_{sim}(s^i_1,t_j) & \text{otherwise},
%\end{array}\right.
%\end{equation}


%We shall begin by describing $p_{corr}$ and then explain the extension to $p^*_{corr}$ for the foreground labelled parts. 
%Note that $\lambda=0.1$ is a balancing coefficient, $p_{corr}$ is the probability of which the two parts correspond, and $p_{sim}$ describes how similar the two parts are.

We compute $p_{corr}(p_1,p_2)$ as follows: 
\begin{equation}
p_{corr}(p_1,p_2) = \frac{N(p_1,p_2)}{ m_{p_2}},
\end{equation}

where $N(p_1,p_2)$ is the number of matching pixels and $m_{p_2}$ is the overall count of pixels in $p_2$. To compute matching pixels, we use the dense correspondence technique of Yoav Ha-Cohen et al. \cite{hacohen2011non} which outputs a confidence value along with the pixel-to-pixel correspondences. We consider matching pixels to be those with confidence values which exceed a certain threshold, which we set empirically to $0.5$. As Figure \ref{fig:NRDC} demonstrates, this yields a rather sparse set of clean correspondences. While other approaches may yield a larger set of correspondences, here we care for precision, or only a small number of false-positive approximate correspondences. 

\section{Pairwise Potentials}

We have three types of pairwise potentials between two different parts in our graph: inter-image potentials $\theta^{corr}_{t_i,t_j}$ and two types of intra-image potentials - $\theta^{source}_{t_i,t_j}$ and $\theta^{sim}_{t_i,t_j}$.

We shall start by defining $\theta^{source}_{t_i,t_j}$ which aims at locating more commonality to the source image than what is evident by the given correspondences. For each source part $s^i_1$, we compute an RGB color histogram and find the $K$ closest parts in the target. We then look at two adjacents parts in the source image and check whether their corresponding parts are also adjacent. If so, we define a pairwise relation as follows:
\begin{equation}
\theta^{source}_{t_i,t_j} = ....
\end{equation}

Rather than allowing any two parts to correspond, we can propagate knowledge from the given pixel correspondences by estimating where the corresponding part in the target should be. We can do so in the following manner: For each part $s^i_1$, we find the closest and furthest foreground corresponding pixels and approximate the location of the corresponding part according to its relative location. We then allow for an uncertainty gap by setting an uncertainty radius according to the distance from the closest correspondence. See Figure \ref{fig:NRDC2} for an illustration.
%We examine if any of the $K$ closest neighbors reside within this \emph{uncertainty area} and update $p_{sim}(s^i_1,t_j)$ accordingly only if one of the $K$ nearest neighbors of one of the template's spatial neighbors is bordering with $t_j$. In other words, we consider target parts that are similar to template parts in pairs. Like with the correspondences, this yields a conservative but highly reliable set....To densify our estimations, we use weaker cues for template foreground parts that have no corresponding pixels. 

Another type of inter-image potential is $\theta^{sim}_{t_i,t_j}$ which measures how likely the two parts coincide, according to the hierarchical segmentation of \cite{arbelaez2011contour}. As parts are defined according to the different thresholds, we can sample various thresholds to compute the likelihood in which two parts will become one according to this method. More precisely, we define a pairwise relation between adjacent parts in each target image according to:
\begin{equation}
\theta^{sim}_{t_i,t_j} = ....
\end{equation}

Pairwise connections between neighbouring images are defined according to the degree of which they correspond. As the dense correspondence technique we use is not symmetric, we define these connections as follows:
\begin{equation}
\theta^{corr}_{t_i,t_j} = \frac{N(t_i,t_j)}{ m_{t_i}}+\frac{N(t_j,t_i)}{ m_{t_j}},
\end{equation}

where $N(t_i,t_j)$ is the number of matching pixels from part $t_i$ to $t_j$ and $m_{t_i}$ is the overall count of pixels in $t_i$.
